SafeBound: A Practical System for Generating Cardinality Bounds

Recent work has reemphasized the importance of cardinality estimates for query optimization. While new techniques have continuously improved in accuracy over time, they still generally allow for under-estimates which often lead optimizers to make overly optimistic decisions. This can be very costly for expensive queries. An alternative approach to estimation is cardinality bounding, also called pessimistic cardinality estimation, where the cardinality estimator provides guaranteed upper bounds of the true cardinality. By never underestimating, this approach allows the optimizer to avoid potentially inefficient plans. However, existing pessimistic cardinality estimators are not yet practical: they use very limited statistics on the data, and cannot handle predicates. In this paper, we introduce SafeBound, the first practical system for generating cardinality bounds. SafeBound builds on a recent theoretical work that uses degree sequences on join attributes to compute cardinality bounds, extends this framework with predicates, introduces a practical compression method for the degree sequences, and implements an efficient inference algorithm. Across four workloads, SafeBound achieves up to 80% lower end-to-end runtimes than PostgreSQL, and is on par or better than state of the art ML-based estimators and pessimistic cardinality estimators, by improving the runtime of the expensive queries. It also saves up to 500x in query planning time, and uses up to 6.8x less space compared to state of the art cardinality estimation methods.

==> response.tex <==
\setcounter{page}{0}

\section*{Response}

We thank the reviewers for providing clear and constructive
instructions.  We have addressed all comments, and significantly
improved the paper.  Some highlights:

\begin{itemize}
  
\item We have extended our experimental evaluation: we extend the PK-FK precomputation to postgres; we added the Simplicity system; we extended the scalability experiments for the construction time; and we communicated with the authors of PessEst to confirm our understanding of that system.  We also made some improvements to our code and reduced the construction time of the statistics on JOBM by 4x and Stats by 6x.  We also improved our code in github.
\item We added a new Sec.~\ref{sec:limitations} {\em Limitations and Future Work} were we discussed limitations and possible extensions of our system.  (We had to eliminate the old Sec. 6 and shortened Sec. 4.3 because of space constraints.)
\item We made several other improvements to the paper; most of them are color coded as specific responses to the reviewers, the minor updates were not color coded.
\end{itemize}

\noindent Note: As we were re-running our experiments, we noticed a small error in result retrieval for PessEst, which affected the results for the JOBM benchmark. We updated the graph and discussion in Sec. 5.
\subsection*{Required Changes by the Metareviewer}

\begin{itemize}
% \item MR1 (PK-FK joins): To test the effect of PK-FK pre-computation in traditional systems, we present another variation on Postgres' estimator called PostgresPK in the relative error experiments. For this version, we pre-computed and materialized the PK-FK joins, resulting in modified FK tables which contain the additional filter columns from the PK tables. Then, we allowed it to generate statistics on these tables and adjusted the queries so that filter predicates on the PK tables now reference the FK table. For example, consider the query $Q(X, A, B) = R(X,A)S(A, B, Y)T(B, Z) \wedge S.Y<10 \wedge T.Z > 5$ where $S.A$ is a PK for $R.A$ and $T.B$ is a PK for $S.B$. We calculate the PK-FK join results $R'(X, A, Y')$ and $S'(A, B, Y, Z')$ and adjust the query to reference them, $Q'(X, A, B) = R'(X, A, Y') S'(A, B, Y, Z') T(B, Z) \wedge R'.Y'<10 \wedge S'.Z' > 5$. This mirrors our method by propagating statistics across PK-FK joins without modifying the query's join graph. We also experimented with applying the filter predicates to both the PK and FK tables, and this produced similar estimates. The alternative methods of PessEst, BayesCard, and NeuroCard already perform similar PK-FK optimizations, so we do not include them in this extension.

\item MR1 (PK-FK joins): We chose option (2) offered by the metareviewer: we extended the experiment in Sec.~\ref{sec:evaluation} (see PostgresPK in Fig. \ref{subfig:relative-error}) to measure the benefit of PK-FK precomputation in Postgres.  See also our response to \revc{R4.O3}.

\item MR2 (Experiments on scalability): As requested, we include additional scale experiments on larger datasets (TPC-H, Scale Factor 1-10).  See the responses to \reva{R1.O1} and \reva{R1.O2}.

\item MR3: Add Simplicity. Done, in Sec. \ref{sec:evaluation}. See response to \revc{R4.O1}.

\item MR4, Clarifications/acknowledgement on how much your proposed heuristics are losing accuracy: Done, in Sec.~\ref{sec:limitations}.  See \revc{R4.O2}.

\item MR5 (Discussion of limitations): Done, as required, in  a new Sec.~\ref{sec:limitations} {\em Limitations and Future Work}.

\item MR6 (Clarify this comment on PessEst): We have communicated with the authors of PessEst, and they have confirmed our understanding: (1) PessEst relies on BoundSketches which store the max degree and cardinality of hash-partitions of the underlying table. This is more detailed than the full-table max degree and cardinality, but ignores any predicates. (2) If the query contains a filter predicate, e.g. "R.A = 5", then PessEst generates a new BoundSketch for affected tables {\bf at query time}, allowing it to account for the lower cardinalities and max degrees caused by the predicate. (3) When the system detects a selective predicate on a PK table, it computes any PK-FK joins {\bf at query time} in order to generate a new bound sketch for the filtered FK table.  Both (2) and (3) occur at query time. Section 3.3 of \cite{DBLP:conf/sigmod/CaiBS19} discusses these techniques; "If a relation is subject to any filter predicates following filter selection propogation, then the BS associated with that relation must be populated at runtime." Additionally, we discuss Chen et al. in Sec.~\ref{sec:intro}.

\item MR7 (R3 and R4 further clarification and writing comments): We appreciated and incorporated the clarification and writing comments.
\end{itemize}


\subsection*{\reva{Required Changes by Reviewer 1}}
\begin{itemize}
\item O1: Construction time. \reva{We demonstrated the scaling of our construction algorithm on a more complex and larger dataset using the TPC-H benchmark in Sec.~\ref{subsec:scalability}.  However, limitations remain: see Sec. \ref{sec:limitations}.  Also, see minor comment in Sec.~\ref{sec:intro}.}
\item O2: $O(n^2)$ degree sequences.  \reva{We discuss this at the end of Sec.~\ref{subsec:choosing:statistics} and provide a fallback method in Sec.~\ref{subsec:cyclic-multi-key}.} 
\item O3: Cyclic queries and beyond.  \reva{We described this in Sec.~\ref{subsec:cyclic-multi-key}; see also minor comment in Sec.~\ref{subsec:problem}.}
\end{itemize}

\subsection*{\revb{Required Changes by Reviewer 3}}
\begin{itemize}
\item O1: Discuss limitations. \revb{Done, in Sec. \ref{sec:limitations}.}
\item O2: Related work. \revb{We add discussion of Chen et al. in Sec.~\ref{sec:intro} and extend the references. Due to space constraints, we could not add a full related works section although we agree that it would be a good addition.}
\item O3: Code provided without instructions. \revb{We significantly expanded the documentation for our code base including scripts for downloading datasets, building data structures, and running experiments. This can be seen in the github repository \cite{github}.}
\end{itemize}

\subsection*{\revc{Required Changes by Reviewer 4}}
\begin{itemize}

\item O1: Add Simplicity. \revc{Done, in Sec. \ref{sec:evaluation}. The open source prototype had several limitations (it was hard coded for the original JOB benchmark and intermingled cardinality estimation with greedy plan enumeration), so we decided to re-implement it for the experiments in Sec. \ref{sec:evaluation}. As in the original code, we combine join columns' max degrees with single-table cardinality estimates from Postgres using their bound. Also, see the clarification of our discussion of previous cardinality bounding systems in Sec \ref{sec:intro}.}
  
\item O2: Assumptions [are] similar to those made by standard statistics. \revc{We clarified this in Sec.~\ref{sec:limitations}.   (See also  minor point in Sec.~\ref{subsec:modeling:cdfs}.)}

\item O3: Benefit of the PK-FK precomputation.  \revc{Done, in Sec.~\ref{sec:evaluation}: see PostgresPK in Fig.~\ref{subfig:relative-error}. We include a comparison with Postgres where it has access to equivalent statistics on the pre-computed PK-FK joins.}
\item O4: Disaggregate the experimental results. \revc{Due to space limitations, we report disaggregated versions of Fig~\ref{fig:Top-80-Runtime}, \ref{fig:Join-Size-Vs-Runtime}, \ref{fig:regressions} in the appendix\cite{github}.}
\item D11, D14, D18, D19: \revc{D11 done in Sec. \ref{subsec:modeling:cdfs}, D14 done in Sec. \ref{sec:evaluation} footnote 4, D19 done in Sec. \ref{subsec:cost}, and the D18 in the appendix \cite{github}.}
\end{itemize}


